Does Human Collaboration Enhance the Accuracy of Identifying LLM-Generated Deepfake Texts?

Advances in Large Language Models (e.g., GPT-4, LLaMA) have improved the generation of coherent sentences resembling human writing on a large scale, resulting in the creation of so-called deepfake texts. However, this progress poses security and privacy concerns, necessitating effective solutions for distinguishing deepfake texts from human-written ones. Although prior works studied humans' ability to detect deepfake texts, none has examined whether "collaboration" among humans improves the detection of deepfake texts. In this study, to address this gap of understanding on deepfake texts, we conducted experiments with two groups: (1) nonexpert individuals from the AMT platform and (2) writing experts from the Upwork platform. The results demonstrate that collaboration among humans can potentially improve the detection of deepfake texts for both groups, increasing detection accuracies by 6.36% for non-experts and 12.76% for experts, respectively, compared to individuals' detection accuracies. We further analyze the explanations that humans used for detecting a piece of text as deepfake text, and find that the strongest indicator of deepfake texts is their lack of coherence and consistency. Our study provides useful insights for future tools and framework designs to facilitate the collaborative human detection of deepfake texts. The experiment datasets and AMT implementations are available at: https://github.com/huashen218/llm-deepfake-human-study.git

==> method_copy.tex <==
% \thai{If space allows, we can add a paragraph that describe the overall idea--i.e., to facilitate user-study via crowdsourcing with both select and write mode + a carefully designed randomized data generation process enabled by GPT-2.}
To improve human performance in deepfake text detection, we first, 
define a realistic problem - detecting deepfake texts in an article authored by both human and an AI (i.e., GPT-2). This is done by randomly replacing 1 out 3 human-written paragraphs with a GPT-2-generated paragraph. Next, we define 2 variables for our study - 
\textit{individual vs. collaboration} and \textit{non-expert vs. expert}. After using these variables to facilitate crowdsourcing recruitment, we ask the human participants to select 1/3 paragraphs that is deepfake and provide justification for selection. 

% \subsection{Problem Formulation}
\begin{figure*}[ht]
    \centering
    % \includegraphics[width=0.9\linewidth]{images/data_process.jpg}
\includegraphics[width=0.9\linewidth]{images/method.pdf}
    \caption{Illustration of the data generation process}
    \label{fig:ntgprocess}
\end{figure*}

\subsection{Data Generation} %\hfill
% Our task is modeled similarly to the \textit{Turing Test} problem defined by Alan Turing in the 1950s. The \textit{Turing Test} is a test administered by a human as the judge who 
% has a conversation with an unknown entity and decides if they are speaking with a human or machine/AI model. If the machine is labeled as human, then the machine has passed the test. 
% However, for our task, due to the security risks deepfake texts pose, it is imperative that 
% the NTG does not pass the test. To that end, we propose a framework that increases the probability of GPT-2 failing the \textit{Turing Test}. 

The goal of distinguishing deepfake texts from human-written texts. As this problem has been studied by several researchers \cite{uchendu2020authorship,clark-etal-2021-thats,ippolito-etal-2020-automatic,dugan2020roft,gehrmann2019gltr} and shown to be very non-trivial and difficult to solve, we 
develop a novel way
of administering the \textit{Turing Test}. 
Thus, we implement a realistic setting of the problem - \textit{detecting deepfake texts in an article authored by both humans and an NTG}. This setting is motivated by the fact that while NTGs currently have very impressive generations, humans still produce more natural speech than NTGs. 
This means that it will be natural for humans to edit machine-generated articles to make them sound more authentic. We study this non-trivial problem by asking human evaluators to: 
(1) Of 3 paragraphs, two written by a human, and one machine-generated, 
select the machine-generated paragraph. 
(2) Please check all explanations that satisfy the reason(s) for your choice. 
See Figure \ref{fig:rqs}(B) for a visual representation of our task. 
We provide seven pre-defined rationales that correspond to flaws typically observed in deepfake text \cite{dou2022gpt}  %\thai{based on which we get these rationales?}
- grammatical issues, repetition, lacks common sense, contains logical errors, contradicts previous sentences, lack of creativity or boring to read, writing is erratic (i.e. does not have a good flow) or choose to write on their own.
% \thai{the previous two paragraphs should be the first paragraph to well motivate this section. Reviewers might already ask why need to go through this complicated process instead of just showing a human-written and a machine-generated article like other works have done. Why our tasks are better fit to study the RQs?}.

To build this dataset, we collected 200 human-written news articles (mostly politics since this work is motivated by mitigating the risk of mis/disinformation or fake news dissemination) from reputable news sources such as CNN and Washington Post. Next, of the 200 articles, we took 
the first suitable 50 articles with at least 3 paragraphs. 
Then, we removed all paragraphs after the 3rd paragraph. Since the goal is to have a multi-authored article (human and AI), we randomly select 1/3 paragraphs to be replaced by GPT-2's \cite{radford2019language} 
generated texts. 
We used only GPT-2 to generate the deepfake texts 
because: (1) GPT-2 and GPT-3 are similar. Based on \cite{uchendu2020authorship, clark-etal-2021-thats}, human performance on detecting GPT-2 and GPT-3 texts have similar 
accuracies; and (2) GPT-2  is cheaper to generate texts with than GPT-3 since GPT-2 is open-source and GPT-3 is not.  For generation, we used GPT-2 XL which has 1.5 billion parameters and \textit{aitextgen}\footnote{https://github.com/minimaxir/aitextgen}, a robust implementation of GPT-2 to generate texts with the default parameters. 
We followed the following replacement process: 
\begin{enumerate}
    \item If paragraph 1 is to be replaced: Use Title as a prompt to generate GPT-2 replacement
    \item If paragraph 2 is to be replaced: Use Paragraph 1 as a prompt to generate GPT-2 replacement
    \item If paragraph 3 is to be replaced: Use Paragraph 2 as a prompt to generate GPT-2 replacement
\end{enumerate}
Since, we are unable to control the number of paragraphs GPT-2
generates given a prompt, we use a Masked Language model to choose the best GPT-2 replacement that fits well with the article. 
We use a BERT-base \cite{devlin2018bert} as the Masked Language model to get the probability of the next sentence. 
Let us call this model G(.), it takes 2 inputs - the first and probable second sentence/paragraph (G($Text\_1, Text\_2$)) and outputs a score. The lower the score, the more probable $Text\_2$ is the next sentence. 

For instance, say GPT-2 texts is to replace Paragraph 2 (P2) of an article
\begin{itemize}
    \item We use P1 as prompt to generate P2 with GPT-2
    \item GPT-2 generates another 3-paragraph article with P1 as the prompt
    \item To find the suitable P2 replacement, we do G(P1, 
    each GPT-2 generated paragraph)
    \item Since low scores with G(.) is considered most probable, the P2 replacement is the 
    GPT-2 paragraph that yielded the lowest score with G(.)
\end{itemize}

We use a random number generator to select which paragraphs are to be replaced and got the following deepfake text replacement for 
the paragraphs in Table \ref{tab:labels}.
After we created these multi-authored articles, we manually did a quality check of 
a few of these articles by checking for consistency and coherence. See Figures  \ref{fig:ntgprocess} for the data generation process and \ref{fig:rqs}(A) for an example of 
the final multi-authored article. 

% \lee{let's make the following argument more visible (eg, title or sub-section) as reviewers will definitely wonder. So, our justification is (1) GPT2 and GPT3 are similar, and (2) GPT2 is chaper. Are there other reasons? Is GPT3 completely open for researchers to access? If so, we can mention it}


% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%     \hline
%        \textbf{Label}  & \textbf{Count}  \\
%        \hline
%        Paragraph 1   &  23 \\
%        Paragraph 2   &  16 \\
%        Paragraph 3   &  11 \\
%        \hline 
%     \end{tabular}
%     \caption{Data labels of deepfake texts}
%     \label{tab:labels}
% \end{table}




\begin{table}[]
\centering
%\footnotesize
\begin{tabular}{r|c|c|c}
\toprule
\cellcolor[HTML]{DAE8FC}\textbf{Label} & \cellcolor[HTML]{DAE8FC}\textbf{Paragraph1} & \cellcolor[HTML]{DAE8FC}\textbf{Paragraph2} & \cellcolor[HTML]{DAE8FC}\textbf{Paragraph3} \\ \midrule
\textbf{Count} & 23                  & 16                  & 11                  \\ 
\bottomrule
\end{tabular}
\caption{Data labels of deepfake texts
%\lee{need to present data in the consistent format. fonts of table 1 are larger than rest of tables}
}
%\vspace{-3em}
\label{tab:labels}
\end{table}




% \begin{figure}[!htb]
% %\small
%   \centering
%   \fbox{%
%     \begin{tabular}{p{0.9\textwidth}}
%     %   \includegraphics[width=0.8\textwidth]{example-image}\\
%       \noindent
% \textbf{Title:} \textit{2 Fort Bliss soldiers in ICU, 9 others hospitalized after ingesting chemical used in antifreeze}
% \\ \hline 
% \small
% The U.S. army statement said the two soldiers received an initial evaluation and additional treatment Friday at the city hospital of El Paso at the soldiers' request.
% \\
% \\
% \small
% The soldiers drank a substance during a field training exercise thinking they were drinking an alcoholic beverage, the statement read, noting alcohol is banned on such exercises. Subsequent toxicology tests revealed the presence of ethylene glycol. Nine other soldiers are also being treated at the hospital in a non-critical care unit as part of the incident.
% \\ 
% \\
% \small
% The circumstances of how the Soldiers ingested the substance are under investigation by the U.S. Army Criminal Investigation Command (USACIDC). There is no reason to believe there is any threat to the greater Fort Bliss community, the statement read.
%     \end{tabular}}
%   \caption{Example of a multi-authored (Human \& GPT-2) 3-paragraphs article}
%   \label{fig:example}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\linewidth]{images/flow_task.jpg}
%     \caption{Task: Detecting deepfake texts}
%     \label{fig:turing}
% \end{figure}
% \subsection{Task} \label{sec:task_description} %\hfill

Next, as we have defined this realistic scenario, we hypothesize that collaboration will improve human detection of deepfake texts. Thus, we define 2 variables for this experiment -
Individual vs. Collaboration and English expert vs. English non-expert. We investigate 
how collaboration (both synchronous and asynchronous) improves from individual-based detection of deepfake texts. The hypothesis here is that when humans come together to solve 
a task, collaborative effort will be a significant improvement from average individual efforts. Additionally, as human detection of deepfake texts is non-trivial, we want to investigate if the task is non-trivial because English non-experts focus on misleading 
cues as opposed to English experts. 

Finally, we observe that based on the replacement algorithm, some 
bias in detection may be introduced. Replacing paragraph 3 may be seen as easier 
because there is no other paragraph after it to judge the coherency. 
However, we keep the generation process fair by only using the 
text right before the paragraph as a prompt to generate the next paragraph. 
Thus, to replace paragraph 3, we only use paragraph 2 as a prompt, not 
the previous paragraphs and title.
% \lee{this will severely undermine the test environment. instead of putting it here, move the paragraph to data generation section, and argue why our generation process is reasonable}


% We follow the reverse of the traditional "Turing Test" format, with the goal of distinguishing machine-generated texts from human-written texts rather than proving NLG models are as smart as humans. Several existing works (e.g., \citet{uchendu2020authorship}, \citet{ippolito-etal-2020-automatic}, \citet{garbacea-etal-2019-judge}) have conducted the evaluations in the context of Turing Test. To achieve this, we provided evaluators with three paragraphs, two written by people and one generated by a model. We then asked two questions: 1) Please select which paragraph is machine-generated; 2) Please check all explanations that satisfy the reason(s) for your choice. The first question is simple, as they must choose only one response. For the second question, on the other hand, evaluators can select one or more responses amongst seven pre-defined rationales (grammatical issues / repetition / lacks common sense / contains logical errors / contradicts previous sentences / lack of creativity or boring to read / writing is erratic (i.e. does not have a good flow)) or choose to write on their own. 


% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.9 \linewidth]{images/instructions.jpg}
%     \caption{AMT Instructions \& Example-based training}
%     \label{fig:instruct}
% \end{figure}








\subsection{Participant Recruitment}
\subsubsection{AMT} 
\label{sec:amt-recruit}

\noindent Inspired by \citet{clark-etal-2021-thats}, \citet{dugan2020roft}, and \citet{van2019best}, we used Amazon Mechanical Turk (AMT) to collect responses from non-expert evaluators. 
We deployed a two-stage process to conduct the non-expert human studies. First, we posted a \emph{Qualification} Human Intelligence Task (HIT) that pays $\$0.50$ per assignment on MTurk to recruit 240 qualified workers
% \thai{Fig. 5 informs that we pay double if the worker selects the correct answer. Should we mention about this as an additional incentive? Should we also mention the approximiate time to finish the task and the estimated wage per hour, compared to federal minimum?}.
% \lee{agree. present basic stat, in the similar wording as Upwork "\$25-\$35 per hours...". CSCW reviewers will be very critical on this, so need to show we paid over min-wage, etc.}
% \hua{Sounds great. the `double-payment' of Fig5 is for the stage describing below. We've added these descriptions in the end of this section.}
In terms of the qualification requirements, in addition to our custom qualification used for worker grouping, three built-in worker qualifications are used in all the HITS, including \emph{i)} HIT Approval Rate (${\leq}98\%$), Number of Approved HITs (${\geq} 3000$), and Locale (US Only) Qualification.
% \thai{shouldn't it be ${\geq}3000$?}\hua{Yes, we've corrected. Thanks!}
% 


Next, we only enable the qualified workers to enter the large-scale labeling tasks.
% we divided the recruited qualified workers into two groups, including an \emph{Individual Group} and a \emph{Collaborative Group}. 
The approximate time to finish each labeling task is around 5 minutes (\ie the average time of two authors on finishing a random HIT). Therefore, we aim for $\$7.25$ per hour and set the final payment as $\$0.6$ for each assignment. Further, we provide ``double-payment'' to workers who made correct submissions as the extra bonus.




\begin{table}[]
%\footnotesize
\begin{tabular}{c|c|c|c}
\toprule
{\cellcolor[HTML]{DAE8FC}\textbf{Participant}} & {\cellcolor[HTML]{DAE8FC}\textbf{Gender}} & {\cellcolor[HTML]{DAE8FC}\textbf{Education}}         & {\cellcolor[HTML]{DAE8FC}\textbf{Group} }              \\ \midrule \midrule
P1          & Female & Bachelor’s degree & \multirow{3}{*}{G1} \\
P2          & Female & Bachelor’s degree &                     \\
P3          & Female & Bachelor’s degree &                     \\ \hline
P4          & Female & Bachelor’s degree & \multirow{3}{*}{G2} \\
P5          & Male   & Bachelor’s degree &                     \\
P6          & Male   & Graduate degree   &                     \\ \hline
P7          & Female & Graduate degree   & \multirow{3}{*}{G3} \\
P8          & Female & Graduate degree   &                     \\
P9          & Female & Bachelor’s degree &                     \\ \hline
P10         & Female & Bachelor’s degree & \multirow{3}{*}{G4} \\
P11         & Female & Bachelor’s degree &                     \\
P12         & Male   & Bachelor’s degree &                     \\ \hline
P13         & Female & Graduate degree   & \multirow{3}{*}{G5} \\
P14         & Female & Bachelor’s degree &                     \\
P15         & Male   & Graduate degree   &                     \\ \hline
P16         & Female & Bachelor’s degree & \multirow{3}{*}{G6} \\
P17         & Male   & Bachelor’s degree &                     \\
P18         & Male   & Bachelor’s degree &                     \\ \bottomrule
\end{tabular}

    \caption{Upwork participant demographics}
    \label{tab:demographics}
\end{table}

\subsubsection{Upwork} 

\noindent We utilized Upwork to recruit expert evaluators, especially those with expertise in writing domains.%\thai{do you mean ``especially those with expertise in writing domains?} 
Upwork is one of the leading freelance websites with a substantial network size: 
Upwork generates 40 million monthly visits on average, and its gross services volume reached 3.5 billion dollars in 2021.\footnote{\url{https://sellcoursesonline.com/Upwork-statistics}} It has facilitated the freelance industry by introducing skilled freelancers in diverse categories like writing, graphic design, and web development. With its automated recommendation system, Upwork is capable of effectively matching clients and workers based on their needs. 

Through Upwork, we first posted a task description as a client to gather participants. We mentioned in the description that this is for research and provided all necessary information such as research objectives and questions we anticipated that they will solve. Our recruitment advertisement also highlighted the mandatory requirements: (1) a participant should be at least 18 years old; and (2) a participant should be a native English speaker. Lastly, if they were willing to proceed, they were asked to submit a proposal answering the following questions: 
(1) what is the highest level of degree you have completed in school? 
(2) did you major in English or English Literature? and 
(3) describe your recent experience with similar projects.  

One useful feature for accelerating the recruitment process in Upwork is that not only workers %\thai{should we use ``workers" instead? ``employees" can be controversal.} 
can apply to the postings but also clients like us can invite prospective candidates that seem suitable for the task to submit proposals. We manually reviewed workers’ profile descriptions who specified their skill sets as copywriting, editing/proofreading, content writing and then sent them invites. 

While making recruitment decisions, we verified participants' eligibility by checking their self-reported age, language, and education in the profile, in addition to evaluating their proposal responses. It resulted in a total of 18 finalists to officially begin the study. Next, we sent them the consent form via the platform's messaging function and activated Upwork contracts only after they returned the signed form. A primary purpose of the contracts was for clients to compensate workers based on submitted hours through the Upwork system. Participants' requested hourly wages ranged from \$25-\$35 per hour depending on their prior experiences and education levels. All 18 individuals successfully signed both documents and were compensated accordingly. Table \ref{tab:demographics} gives the self-reported demographic breakdown of recruited Upworkers.







\begin{figure*}[!t]
    \centering
    % \includegraphics[width=0.9 \linewidth]{images/task1.jpg}
    \includegraphics[width=0.9 \linewidth]{images/task11.pdf}
    \caption{User Interface for the AMT Collaborative Group workers to choose the machine-generated paragraph.}
    \label{fig:task1}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/introduction.pdf}
    \caption{The instructions to train users by providing prompt feedback.}
    \label{fig:question type2}
\end{figure*}


\subsection{Experiment Design}
\subsubsection{AMT} 
\label{sec:amt-expt}
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%     \hline
%       \textbf{Individual}   & \textbf{Collaboration} \\
%       \hline 
%         Select & Select \\
%         Write & Write \\
%         \hline 
%     \end{tabular}
%     \caption{AMT question types for each setting}
%     \label{tab:scenario}
% \end{table}



\begin{figure}
    \centering
    % \includegraphics[width=0.9 \linewidth]{images/select.jpg} \hfill
    % \includegraphics[width=0.9 \linewidth]{images/write.jpg}
    \includegraphics[width=\linewidth]{images/step2.pdf}
    \caption{\emph{Select} (A) vs. \emph{Write} (B) justification question type}
    \label{fig:question type1}
\end{figure}


\noindent During the large-scale labeling task, we divide the recruited qualified workers into two groups to represent the individual vs. collaborative settings, respectively. We define group1 as \emph{Individual Group}, in which each worker was asked to select the machine-generated paragraph 
without any references. See Figure~\ref{fig:task1}, for example, humans in \emph{Individual Group} can only see the introduction with panel (A) (B) and (C).
On the other hand, we design the group 2 to be \emph{Collaborative Group}, where the workers were asked to conduct the same task after the \emph{Individual Group} finishes all HITs (\ie see panel (A), (B), (C) in Figure~\ref{fig:task1}). In addition, workers from the \emph{Collaborative Group} could also see the selection results from the group1 in an asynchronously manner, as the example shown in Figure~\ref{fig:task1}(D), to support their own selection. 

In addition, we investigate the 
capability of Individual vs. Collaboration of non-expect 
human participants to 
improve human performance in deepfake text detection. 
% To do this, 
% we compare  2 ways the human participants can provide justification for their answer - \textit{Select} \& \textit{Write}. 
Next, we build the justification part similar to  RoFT \cite{dugan2020roft}, a gamification technique for improving human performance in deepfake text detection.
In the RoFT framework, participants were asked to select from a pre-defined list one or more reasons such as repetition, grammar errors, etc. Participants were also
given another option, where they can enter their own justification if they do not find any suitable selection from the provided list. 

% \hua{Added incentives settings and cost.}
Furthermore, we take actions to incentivize workers to provide qualified results: \emph{i)} in our instruction, we provide immediate feedback on the worker's selection to calibrate their accuracy. In specific, after reading the HIT instruction (\ie Figure~\ref{fig:question type2} (A)), workers can get a deeper understanding of ``which paragraph is generated by AI machine'' by trial and error on selecting one example (\ie Figure~\ref{fig:question type2} (B)). Participants were given unlimited chances to change their answers. This example-based training process was inspired by \citet{clark-etal-2021-thats}'s human evaluation study and was found to be the most effective 
training technique. \emph{ii)} We pay double compensations to the workers who provide correct answers as mentioned in Section~\ref{sec:amt-recruit}. This aims to encourage workers to get high accuracy on selecting the correct machine-generated paragraphs. \emph{iii)} We set the minimum time constraint (\emph{i.e.,} one minute) for workers to submit their HITs, so that the workers will concentrate on the task for at least one minute instead of randomly selecting one answer and submitting the HIT. Note that we also disabled the copy and paste functions in the user interface to prevent workers from searching for the paragraphs from online resources.

% 

% Next, for all settings, we first provided an example of a human-written paragraph vs. a machine-generated paragraph to train participants on the task (Figure \ref{fig:question type2}). Participants were given unlimited chances to change their answers. This example-based training process was inspired by \citet{clark-etal-2021-thats}'s
% human evaluation study and was found to be the most effective 
% training technique. 
% % See figure 
% \ref{fig:instruct} for instructions and example-based framework.






\subsubsection{Upwork} 
Given that we aim to compare experts' deepfake text detection accuracy with respect to individual vs. collaborative settings, our Upwork study consists of two sub-experiments. 
The first experiment asks Upwork participants to perform a given task on their own. The second experiment requires three individuals to solve the questions as one group in a synchronous manner.

We used Qualtrics\footnote{\url{https://www.qualtrics.com}} service to generate and disseminate the study form. The user interface was equivalent to the \emph{select} scenario in Figure \ref{fig:question type1}. Upwork participants were given one week to complete the survey. Upon completion, we randomly grouped 3 participants per team, resulting 6 teams in total for synchronous collaboration (Table \ref{tab:demographics}). All discussions were conducted on the video communications software - Zoom\footnote{\url{https://zoom.us}} and we leveraged Zoom's built-in audio transcription feature, which is powered by Otter.ai\footnote{\url{https://otter.ai}} for discourse analyses. In addition to the written consent obtained during the recruitment procedure, verbal consent for participation in the discussion and for audio recording was obtained prior to the start of each session. One member of the study team served as a moderator for the meetings. Depending on the participant's schedule and level of commitment in their group, each meeting lasted 1.5 - 3 hours. 


\subsection{Evaluation: Performance Measurement}
We measure how well participants perform the tasks and compared them across different experiment settings. To quantify the detection performance of each setting, we computed the proportion of people who got the answer correct given a set of 50 questions $Q$=\{$q_1$, $q_2$,..., $q_{50}$\}. Suppose $l_n$ is the number of participants with correct answers, and $m_n$ is the total number of participants for the question $q_n$, we calculated the accuracy using this formula: $acc_n$ =$l_n$/$m_n \times 100$. This resulted in a list of accuracy scores $ACC$=\{$acc_1$, $acc_2$, ..., $acc_{50}$\}, representing the participants' performance of 50 articles. To further evaluate whether the means of two groups (individual vs. collaborative \& non-experts vs. experts settings) are statistically different, we conducted a paired independent sample T-test. %This article-level test has a sample size equivalent to the total number of articles (n=50). The values for comparison are computed by taking the average performance of participants per article. 
Since the T-test is grounded on the assumption of normality \cite{gerald2018brief}, we ran the Kolmogorov-Smirnov test on our data and confirmed that the requirement was satisfied. Following, we summarize the results of statistical testing.



\begin{table}[!htb]
\footnotesize
    \centering
    \begin{tabular}{c|c|c}
    \toprule
    SETTING     &    Mean Accuracy                &  p-value  \\                                                
                                  \midrule \midrule
    Baseline vs. Individual      & \multicolumn{1}{c|}{33.33\% vs. 44.99\%}    &  3.8e-05 \\ \hline
    Baseline vs. Collaboration   & \multicolumn{1}{c|}{33.33\% vs. 51.35\%}    &  2.8e-05 \\ \hline
    Individual vs. Collaboration & \multicolumn{1}{c|}{44.99\% vs. 51.35\%} &  0.054    \\ \bottomrule
    \end{tabular}
    \caption{Paired T-test Results for AMT Experiments (RQ1)}
    \label{tab:rq1_amt}
\end{table}



\begin{table}[!htb]
\footnotesize
    \centering
    \begin{tabular}{c|c|c}
    \toprule
    SETTING     &    Mean Accuracy                &  p-value  \\                                                
                                  \midrule \midrule
    Baseline vs. Individual      & \multicolumn{1}{c|}{33.33\% vs. 56.11\%}    &  8.2e-11 \\ \hline
    Baseline vs. Collaboration   & \multicolumn{1}{c|}{33.33\% vs. 68.87\%}    &  1.2e-12 \\ \hline
    Individual vs. Collaboration & \multicolumn{1}{c|}{56.11\% vs. 68.87\%} &  1.3e-05    \\ \bottomrule
    \end{tabular}
    \caption{Paired T-test Results for Upwork Experiments (RQ1)}
    \label{tab:rq1_Upwork}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% %\footnotesize
% \centering
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{c|cc|cc}
% \toprule
% \multirow{2}{*}{SETTING}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Select}}                                                    & \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Write}}                                                    \\ \cmidrule{2-5} 
%                                                                                       & \multicolumn{1}{c|}{Mean Accuracy}                &  p-value  & \multicolumn{1}{c|}{MeanAccuracy}                &  p-value \\ \midrule \midrule
% \begin{tabular}[c]{@{}c@{}}AMT-Individual \\  vs. Upwork-Individual\end{tabular}       & \multicolumn{1}{c|}{44.99\% vs. 56.11\%} &  0.002   & \multicolumn{1}{c|}{45.92\% vs. 56.11\%} &  0.028 \\ \hline
% \begin{tabular}[c]{@{}c@{}}AMT-Collaboration\\  vs. Upwork-Collaboration\end{tabular} & \multicolumn{1}{c|}{51.35\% vs. 68.87\%}      & 1.1e-05 & \multicolumn{1}{c|}{51.97\% vs. 68.87\%}        & 0.003 \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
%     \caption{Paired T-test Results for AMT vs. Upwork (RQ2)}
%     \label{tab:rq2_Upwork}
% \end{table*}


